Social Signal Bench: Evidence-Weighted Evaluation of Co-occurring Social Signals in Video and Audio

Recognizing social signals such as interest and hesitation requires interpreting context-dependent behaviors that may co-occur in conversation. Existing affective computing benchmarks rarely evaluate such co-occurring signals, and conventional multi-label F1 overlooks semantic relationships and annotator disagreement. We introduce Social Signal Bench, a 47-hour densely annotated benchmark for the evaluation of social signal recognition and engagement, comprising two datasets: Social Signal Bench Video (25 hours), covering ten social signals in audiovisual recordings, and Social Signal Bench Audio (22 hours), covering six signals in audio-only recordings. Each dataset pairs a public training set of online conversational video, of which 10 hours are expert-annotated and the remainder pseudo-labeled, with a private expert-labeled test set spanning four conversational domains. We also propose Evidence-Weighted F1 (EW-F1), which weights reference labels by annotator evidence and assigns graded credit to semantically related predictions through optimal per-clip matching. Controlled perturbations demonstrate that EW-F1 distinguishes semantically related errors from unrelated ones, unlike conventional F1. Under a shared evaluation protocol, 7B open models post-trained on Social Signal Bench outperform general-purpose frontier models on video and match them on audio.

==> figures/teaser_v2_annotations.tex <==
\def\TeaserRaterSpans{9.500/16.167/1/0/1, 9.750/20.333/2/0/1, 43.292/55.167/2/0/1, 16.125/21.542/3/0/1, 36.417/43.292/3/0/0.66, 20.375/29.167/4/0/1, 21.083/29.208/4/1/1, 25.000/29.625/4/2/0.66, 36.500/40.708/4/0/1, 37.500/41.667/4/1/1, 37.542/42.375/4/2/1}
\def\TeaserSlices{9.500/16.167/1/1, 9.750/20.333/2/1, 43.292/55.167/2/1, 16.125/21.542/3/1, 36.417/43.292/3/0.66, 20.375/25.000/4/1, 25.000/29.167/4/0.999, 29.167/29.208/4/0.971, 29.208/29.625/4/0.66, 36.500/42.375/4/1}
\def\TeaserWeights{1/1.00, 2/1.00, 3/0.81, 4/0.99}

